Channel Responses for the Molecule Release from Spherical Homogeneous Matrix Carriers

Molecular communications is a promising framework for the design of controlled-release drug delivery systems. Under this framework, drug carriers, diseased cells, and the channel are modeled as transmitters, absorbing receivers, and diffusive channel, respectively. In this paper, we investigate diffusion-based spherical matrix-type drug carriers, which are employed in medical applications. In a matrix carrier, the drug molecules are dispersed in the matrix core and diffuse from the inner to the outer layers of the carrier once immersed in a dissolution medium. We derive the channel response of the matrix carrier transmitter for an absorbing receiver and compare our results with commonly used point and transparent spherical transmitters to highlight the necessity of considering practical models. Furthermore, we derive a criterion for evaluating whether the release process or the channel dynamics are more important for the characteristics of the channel response of a drug delivery system. For the limiting regimes, where only the release process or the channel determine the behavior of the end-to-end system, we propose closed-form approximations for the channel response. Finally, we investigate the channel responses for the release of common therapeutic drugs, e.g., doxorubicin, from a diblock copolymer micelle acting as drug carrier.

==> eval.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.9\linewidth]{./fig/fig_impulse/linear-imp}
	\caption{impulse response for absorbing and passive RX at $d = 2\si{\micro\meter}$}
	\label{fig:4}
\end{figure}


\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{\linewidth}
            \centering
            	\includegraphics[width=\linewidth]{./fig/deviation/deviation_abs_2}
            	\vspace{-3ex}
            \caption{Absorbing RX}
    \label{fig:5:a}
    \end{subfigure}\\
    \begin{subfigure}[b]{\linewidth}
            \centering
            \includegraphics[width=\linewidth]{./fig/deviation/deviation_pas_2}
            	\vspace{-3ex}
            \caption{Passive RX}
    \label{fig:5:b}
    \end{subfigure}    

 	\caption{Deviation of proposed drug release and volume release from \cite{noel:16} for different $\acs$ values.}
 	\label{fig:5}
 \end{figure}


%\begin{figure*}
%	\includegraphics[width=\linewidth]{./fig/fig_log/log-imp}
%	\caption{}
%	\label{fig:3}
%\end{figure*}






==> real_param.tex <==
%\begin{figure*}
%	\centering
%	\includegraphics[width=0.8\linewidth]{./fig/nanogels_v1}
%	\caption{Nanogels bla bla bla}
%	\label{fig:nanogel}
%\end{figure*}
In the previous section we discussed different models for the release of molecules from homogeneous non-erodible matrix systems. 
%
The main goal of these models is their application to realistic DD systems, i.e., they should be able to characterize the behavior of realistic drug carriers.
% 
In the following we introduce an example for the release of different drug molecules from a realistic drug carrier. 

In most studies of practical drug carriers, heuristic models are employed (cf., \cite{Macha_20, Siepmann2008, Arifin2006}), where measurement data are fitted to a mathematical model with several degrees of freedom. 
%
The reason why more elaborate models, as discussed in Section~\ref{sec:drug}, are rarely applied is that it is cumbersome to estimate values for the parameters.
%, e.g., $\nacs$, $\Dm$. 
Nevertheless, the application of more complex models is desirable, as they provide a direct relation between the amount of released drug $M$ and physical parameters of the drug and the carrier and, thus, give important insight into the release process. 
In \cite{Sutton2007}, the parameters for a similar model as discussed in Section~\ref{sec:drug} have been estimated from measurements of the release process of different drug molecules from diblock copolymer micelles, acting as practical homogeneous matrix system.
%
Therefore, we want to employ the practical drug carriers investigated in \cite{Sutton2007}. In particular,  
we use the estimated parameter values in Section~\ref{sec:eval} to analyze the CR for practical drug carriers and molecules.

\subsection{Drug Carrier and Drug Molecules}
\begin{table*}[t]
\caption{\small Parameter values for DOX and $\beta$-lap loaded in the micelle core \cite{Sutton2007}.}
\label{tab:acs}
\centering
\begin{tabular}{p{2.6cm}p{2cm}p{1cm}p{3cm}}
\hline\noalign{}
Drug molecule & $A$ in $\si{\milli\gram\per\milli\liter}$& $\nacs$ &$\Dm$ in $\si{\square\meter\per\second}$\\
\noalign{\smallskip}\hline\noalign{\smallskip}
Doxorubicin (DOX)  & &&\smallskip\\
pH~$5.0$  & $47.5$& $63.7$ & $1.82\cdot 10^{-22}$	\smallskip\\
pH~$7.4$ & $47.5$& $757.5$ & $1.82\cdot 10^{-22}$\\
\noalign{\smallskip}\hline\noalign{\smallskip}
$\beta$-lapachone ($\beta$-lap) & $14.1$ & $370.4$ & $2.42\cdot 10^{-21}$ 	\smallskip\\
\noalign{\smallskip}\hline\noalign{\smallskip}
\end{tabular}
\vspace*{-4ex}
\end{table*}
%\begin{figure*}
%	\centering
%	\includegraphics[width=0.4\linewidth]{fig/micelle}
%	\vspace*{-2ex}
%	\caption{\small Schematic of a diblock copolymer micelle. The micelle core consists of poly(ethylene glycol)-b-poly($_\mathrm{D,L}$-lactide) (PLA) and surrounded by the corona consisting of poly(ethylene glycol) (PEG). The drug molecules (red circles) are either $\beta$-lapachone or doxorubicin molecules \cite{Sutton2007}.}
%	\label{fig:micelle}
%\end{figure*}

As drug carriers, we consider diblock copolymer micelles, efficient drug carriers that have reached clinic trials in several cases \cite{Sutton2007}. 
Furthermore, micelles exhibit a lot of properties beneficial for efficient DD, i.e., increased drug solubility, passive tumor targeting, and several functionalizations \cite[Fig.34-d]{Chude_Okonkwo_19}, \cite{Sutton2007, Ahmad2014}. 
A schematic illustration of a loaded diblock copolymer micelle is shown in Fig.~\ref{fig:micelle}.
The micelle core of radius $a\approx 4.5\si{\nano\meter}$ is made of poly(DL-lactide) (PLA), where drug molecules are homogeneously distributed inside \cite{Sutton2007}. 
The micelle core is surrounded by a polymer corona block made of poly(ethylene glycol) (PEG). 
The influence of the corona on the drug release kinetics is neglected for the derivation of a CR in this paper, i.e., once a drug molecule is released from the core matrix of the micelle, it is not further influenced by the corona and can diffuse freely in the channel. 

As drug molecules we consider $\beta$-lapachone ($\beta$-lap) and doxorubicin (DOX), one of the most common chemotherapeutic drugs \cite{Sutton2007,Weinberg2007}. 
The relevant model parameters for both drug molecules, estimated in \cite{Sutton2007}, are summarized in Table~\ref{tab:acs}. 
As the solubility $C_\mathrm{s}$ of DOX, in contrast to $\beta$-lap, exhibits a dependency on the pH value of the surrounding medium, different $\nacs$-values are considered to observe the release of DOX at different pH levels. 
In particular, we consider a pH value of $5$ that is characteristic for tumor cells, while in blood vessels a pH of $7.4$ is reasonable \cite{D0BM01729A}.
%
From Table~\ref{tab:acs} we observe that the diffusion coefficients $\Dm$ are rather small, as the drug molecules diffuse very slow inside the micelle core\footnote{Since these values have been estimated from real measurements in \cite{Sutton2007}, they may reflect the influence of several physical and chemical effects that slow down the diffusion of drug molecules inside the micelle core.}.  
We note that there are also several time-dependent effects that occur during the release process, e.g., DOX molecules start to interact with the polymer, which further influence the release process. 
As previously mentioned, we neglect long-term interactions between the polymer and the drug molecules in this paper. 



==> tikzlibrarydsp.code.tex <==
% -------------------------------------------------------------------------
% This library for block diagrams and signal flow graphs was inspired by
% the library "signalflow" of Dr. Karlheinz Ochs, Ruhr-University of Bochum,
% Germany. Furthermore, some ideas were taken from the library "circuitikz"
% of Massimo A. Redaelli and from the PGF library itself.
%
% Copyright 2012 by Matthias Hotz
%
% This work is licensed under the Creative Commons Attribution 2.5 Generic
% License. To view a copy of this license, visit
%          http://creativecommons.org/licenses/by/2.5/
% or send a letter to Creative Commons, 444 Castro Street, Suite 900,
% Mountain View, California, 94041, USA.
% -------------------------------------------------------------------------

\usetikzlibrary{arrows, calc, positioning, decorations.markings}

% -------------------------------------------------------------------------
% Parameters for the library

\newcommand{\dsplinewidth}{0.25mm}           % Line width for connections
\newcommand{\dspblocklinewidth}{0.3mm}       % Line width for blocks
\newcommand{\dspoperatordiameter}{4mm}       % Diameter for adder, multiplier, mixer
\newcommand{\dspoperatorlabelspacing}{2mm}   % Distance from symbol to label for adder, multiplier, mixer
\newcommand{\dspnoderadius}{1mm}             % Filled and empty node
\newcommand{\dspsquareblocksize}{8mm}        % Size for square blocks, e.g. for delay elements, decimator, expander
\newcommand{\dspfilterwidth}{14mm}           % Width of a filter block

% -------------------------------------------------------------------------
% Define new arrow heads

\pgfarrowsdeclare{dsparrow}{dsparrow}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt} % Solid line (do not dash)
	\pgfsetmiterjoin	 % Fixed miter join of line
	\pgfsetbuttcap		 % Fixed butt cap of line
	\pgfpathmoveto{\pgfpoint{-4\arrowsize}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{4\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{-4\arrowsize}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

\pgfarrowsdeclare{dsparrowmid}{dsparrowmid}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt}
	\pgfsetmiterjoin
	\pgfsetbuttcap
	\pgfpathmoveto{\pgfpoint{0}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{8\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{0}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

% -------------------------------------------------------------------------
% Define new node shapes

\makeatletter

\pgfkeys{/tikz/dsp/label/.initial=above}

% Generic shape generator for operators, i.e. nodes with a circular
% shape with an additional customizable drawing and a text label
\long\def\dspdeclareoperator#1#2{
	\pgfdeclareshape{#1}
	{
		% Saved anchors, macros and dimensions
		\savedanchor\centerpoint{\pgfpointorigin}
		\savedmacro\label{\def\label{\pgfkeysvalueof{/tikz/dsp/label}}}
	  \saveddimen\radius
	  {
		  \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
		  \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
	    \ifdim\pgf@xa>\pgf@ya
	      \pgf@x=.5\pgf@xa
	    \else
	      \pgf@x=.5\pgf@ya
	    \fi
	  }
	  
	  % Inherit all anchors from the 'circle'-shape:
	  \inheritanchor[from={circle}]{center}
	  \inheritanchor[from={circle}]{mid}
	  \inheritanchor[from={circle}]{base}
	  \inheritanchor[from={circle}]{north}
	  \inheritanchor[from={circle}]{south}
	  \inheritanchor[from={circle}]{west}
	  \inheritanchor[from={circle}]{east}
	  \inheritanchor[from={circle}]{mid west}
	  \inheritanchor[from={circle}]{mid east}
	  \inheritanchor[from={circle}]{base west}
	  \inheritanchor[from={circle}]{base east}
	  \inheritanchor[from={circle}]{north west}
	  \inheritanchor[from={circle}]{south west}
	  \inheritanchor[from={circle}]{north east}
	  \inheritanchor[from={circle}]{south east}
	  \inheritanchorborder[from={circle}]
	  
	  % Draw circle and embed additional code
	  \backgroundpath
	  {
	    % Draw circle
	    \pgfpathcircle{\centerpoint}{\radius}
	    
	    % Embed additional code
	    % (Note that this code must call e.g. \pgfusepathqstroke
	    #2
	  }
	
		% Define anchor parametrized by the PGF key /tikz/dsp/label
	  \anchor{text}
	  {
			\centerpoint
			%
	    \def\templabelabove{above}
	    \def\templabelbelow{below}
	    \def\templabelleft{left}
	    \def\templabelright{right}
	    \pgfutil@tempdima=\dspoperatorlabelspacing
	    %
	    \ifx\label\templabelabove
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by \radius
				\advance\pgf@y by \pgfutil@tempdima
	    \fi
	    %
	    \ifx\label\templabelbelow
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by -\radius
				\advance\pgf@y by -\pgfutil@tempdima
				\advance\pgf@y by -\ht\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelleft
				\advance\pgf@x by -\radius
				\advance\pgf@x by -\pgfutil@tempdima
				\advance\pgf@x by -\wd\pgfnodeparttextbox
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelright
				\advance\pgf@x by \radius
				\advance\pgf@x by \pgfutil@tempdima
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	  }
	}
}

\dspdeclareoperator{dspshapecircle}{\pgfusepathqstroke}

\dspdeclareoperator{dspshapecirclefull}{\pgfusepathqfillstroke}

\dspdeclareoperator{dspshapeadder}{
	% Coordinate offset for the plus
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.55\pgfutil@tempdima
	
	% Draw plus
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{0pt}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{0pt}}}
	
	\pgfusepathqstroke
}

\dspdeclareoperator{dspshapemixer}{
	% Coordinate offset for the cross
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.707106781\pgfutil@tempdima
	
	% Draw cross
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{ \pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{-\pgfutil@tempdima}}}
	
	\pgfusepathqstroke
}

\makeatother

% -------------------------------------------------------------------------
% Define node styles

\tikzset{dspadder/.style={shape=dspshapeadder,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmultiplier/.style={shape=dspshapecircle,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmixer/.style={shape=dspshapemixer,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}

\tikzset{dspnodeopen/.style={shape=dspshapecircle,line width=\dsplinewidth,minimum size=\dspnoderadius}}
\tikzset{dspnodefull/.style={shape=dspshapecirclefull,line width=\dsplinewidth,fill,minimum size=\dspnoderadius}}

% The fixed specification of text height and text depth is the somewhat
% unaesthetic workaround to align the text in different node at the same
% baseline. See the PGF/TikZ manual, ch. 5.1.
\tikzset{dspsquare/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum size=\dspsquareblocksize}}
\tikzset{dspfilter/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum height=\dspsquareblocksize,minimum width=\dspfilterwidth}}

% -------------------------------------------------------------------------
% Define "signal flow" lines

\tikzset{dspline/.style={line width=\dsplinewidth},line cap=round,line join=round}
\tikzset{dspconn/.style={->,>=dsparrow,line width=\dsplinewidth},line cap=round,line join=round}%line cap=rect,line join=miter}
\tikzset{dspflow/.style={line width=\dsplinewidth,line cap=round,line join=round,
  decoration={markings,mark=at position 0.5 with {\arrow{dsparrowmid}}},postaction={decorate}}}

% -------------------------------------------------------------------------
% Define various utility macros

\newcommand{\downsamplertext}[1]{\raisebox{0.1em}{$\big\downarrow$}#1}
\newcommand{\upsamplertext}[1]{\raisebox{0.1em}{$\big\uparrow$}#1}

